A Dataset and Benchmarks for Multimedia Social Analysis

We present a new publicly available dataset with the goal of advancing multi-modality learning by offering vision and language data within the same context. This is achieved by obtaining data from a social media website with posts containing multiple paired images/videos and text, along with comment trees containing images/videos and/or text. With a total of 677k posts, 2.9 million post images, 488k post videos, 1.4 million comment images, 4.6 million comment videos, and 96.9 million comments, data from different modalities can be jointly used to improve performances for a variety of tasks such as image captioning, image classification, next frame prediction, sentiment analysis, and language modeling. We present a wide range of statistics for our dataset. Finally, we provide baseline performance analysis for one of the regression tasks using pre-trained models and several fully connected networks.

==> extra.tex <==
 

% There have been a number of large datasets that are focused on vision and language, however many of these datasets contain only a few modalities compared to the data that we present here.

% \indent Video to sentiment prediction (https://arxiv.org/pdf/1806.06176.pdf). All datasets are videos with annotations for sentiment. (https://arxiv.org/pdf/1808.03920.pdf) Uses a subset of datasets from the paper above and achieved better sentiment predictions

% \indent Sequence to sequence, but did 1 to k, k to 1, and k to k experiments. Dataset are WMT'15, newstest2013, newstest2014, and newstest2015, which are purely NLP and has no vision parts (https://arxiv.org/abs/1511.06114)

% \indent Sequence to tagging, chunking, Dependency Parsing, semantics relatedness, and textual entailment (https://arxiv.org/pdf/1611.01587.pdf). Uses Wall Street Journal (WSJ) portion of Penn Treebank (annotates syntactic or semantic sentence structure) as the dataset for the first three tasks, and SICK dataset for the other two tasks (https://www.aclweb.org/anthology/S14-2001.pdf [about 10,000 English
% sentence pairs annotated for relatedness in meaning and entailment])

% \indent One model to learn them all \cite{kaiser2017one} uses MS-COCO, ImageNet, WSJ parsing dataset, WSJ speech corpus, WMT English-German/French translation corpus and their reverses (8 encoders and decoders in total). k to k experiments with both vision and NLP. Performed ImageNet top-5 accuracies and BLEU for WMT English-German/French translations, with other experiments. \textcolor{red}{(Maybe we can use their image and language modalities' encoders???)}

% \indent (https://ai.googleblog.com/2018/09/conceptual-captions-new-dataset-and.html)
% Google Conceptual Captions Dataset is a 3.3M image/caption pair generated through data over the web. 
% Similarities: contains images and captions, presumably our range of variety is not too far off (can't tell)
% Differences: Google's dataset replaces all specific names/places with conceptual names (Italian cuisine --> cuisine, Dancing in LA --> Dancing, Elvis Presley --> singer, etc). It has 16K "concepts" (i.e. generic words), each of which is mentioned for at least 100 times (we just select the 1000 top used tags). Our dataset has more modalities (video, title, comments), is more interactive (i.e. so many comments), and multiple images to one title and multiple tags instead of one image to one caption

% \indent (http://cocodataset.org/home)
% MS-COCO is a 328K images dataset, containing segmented \& labeled objects. On average each image contains 7.7 object instances, for a total of 2.5M object instances.
% Similarities: contains images
% Differences: MS COCO largely focus on providing non-iconic (partially occluded, in the background, etc), multi-object per image, and segmented objects in each image. Out dataset has more modalities (video, title, comments, tags), have a combination of objects and texts in the image/video, and multiple image/video corresponding to one tag.

% \textcolor{red}{TODO: Compare and contrasts our dataset with other's}


% \iffalse
% Two survey sites:
% https://github.com/artix41/awesome-transfer-learning#deep-transfer-learning
% http://johnarevalo.github.io/2015/02/18/multimodal-datasets.html

% # https://www.reddit.com/r/datasets/comments/3bxlg7/i_have_every_publicly_available_reddit_comment/ 
% This is the most popular Reddit dataset on Kaggle. It contains 1.7B reddit comments, spanning from October 2007 to May 2015
% Similarities: contains comment trees
% Differences: Their dataset is huge. Comments in Imgur (up, down, points, platform) has different properties than those in Reddit (score, edited, up, down, link), but in general Reddit dataset has wider range of categories in terms of comments. However, our dataset contains images, videos, title (Not sure this is unique to our dataset), tags, img_description. Our dataset has more modalities. [Reddit has posts with images, but I can't find a popular one that is highly used. It has the potential to generate a dataset like ours]
% https://www.ceid.upatras.gr/webpages/faculty/zaro/teaching/alg-ds/PRESENTATIONS/PAPERS/2019-Radford-et-al_Language-Models-Are-Unsupervised-Multitask-%20Learners.pdf
% OpenAI dataset "WebText", consisting of texts from all outbound links from Reddit (excluding Wikipedia links) that received at least 3 karma. The actual dataset is https://github.com/jcpeterson/openwebtext

% # https://www.kaggle.com/electron0zero/giphy-dataset
% Giphy dataset contains links for 10k gifs from giphy.com
% Similarities: some of our posts also contain gifs/videos
% Differences: We have more modalities, and some of the images/videos/gifs contain descriptions

% # https://snap.stanford.edu/data/twitter7.html
% # https://dataverse.harvard.edu/dataset.xhtml?persistentId=doi:10.7910/DVN/PDI7IN
% Various datasets are available for twitter. The Stanford one has 467M tweets and is used in one paper (2009), while the Harvard one is about 280M tweets
% Similarities: time/date, content
% Differences: Their dataset is huge. we have more modalities. It seems that most twitter dataset lacks images/videos/gifs. [Although twitter has the potential to generate one like ours]

% # https://vcl.iti.gr/dataset/i-search-multimodal-dataset/ 
% A 10305 objects dataset that uses images, 3D objects, videos, sounds, text or their combinations to query any or a combination of them (Audio and video are mostly not present)
% Similarities: share most of the modalities
% Differences: our dataset is significantly larger (current estimate around 0.3M to 0.4M). We have image description, tag,s and comments, but they have audio.

% # https://ieee-dataport.org/documents/multimodal-dataset-instragram
% 56861 microblogs from instagram containing both images and texts. The dataset was scraped based on 97 hashtags of "Top 100" on Instagram.
% Similarities: Both contains images and texts
% Differences: Our dataset is significantly larger. Their dataset is more uniform as they drop ones without texts. Our dataset contains more modality (video, comments, etc)

% # http://www.cs.cmu.edu/~pliang/papers/acl2018_mosei.pdf (This paper provides basic survey of other datasets)
% # https://www.amir-zadeh.com/datasets
% CMU-MOSEI contains 65+ hours of annotated video (23453 video segments) from 1000+ speakers and 250 topics. It includes texts (manual transcription aligned with audio to phoneme level), videos, and audio. 
% Similarities: Shares some of the modalities.
% Differences: They include sentiment analysis and emotion recognition. Their dataset has greater emphasis on correlating language (text) with audio (speaking voices) and video (expressions, enunciation, etc.). Our dataset has a greater focus over social interactions between and the cultural values within a group of people. We also have comments, a response to a source of information, instead of just the source itself.




% Less relevent datasets:
% https://arxiv.org/pdf/1910.06078.pdf    time-synchronized multimodal data records of students (learning logs, videos, EEG brainwaves) as they work in various subjects from Squirrel AI Learning System (SAIL) to solve problems of varying difficulty levels. 
% https://ieee-dataport.org/open-access/create-multimodal-dataset-unsupervised-learning-and-generative-modeling-sensory-data    all data measurements from a floor cleaning robot



% ##########################################################################
% https://arxiv.org/ftp/arxiv/papers/1803/1803.01164.pdf
% Sucrvey paper on deep learning methods

% https://arxiv.org/pdf/1806.08730.pdf
% decaNLP challenge that contains ten NLP tasks, and MQAN (Multitask Question Answering Network) that jointly learns all tasks in decaNLP without any task-specific modules or parameters.

% http://papers.nips.cc/paper/7334-multi-task-learning-as-multi-objective-optimization.pdf
% Optimize over multi-task learning. Came up with MGDA-UB problem (Multiple Gradient Descent Algorithm – Upper Bound), with the overall objective of finding a Pareto optimal
% solution

% https://dl.acm.org/doi/abs/10.1145/3205455.3205489
% architecture search for multitask networks

% https://www.mitpressjournals.org/doi/pdf/10.1162/tacl_a_00017
% A Multi-Task Learning algo that transforms from Syntax intertwined with translation to pure Translation

% https://arxiv.org/pdf/1904.09751.pdf
% Decoding strategy for text modalities to increase richness of decoded text

% https://icml.cc/2011/papers/399_icmlpaper.pdf
% bimodel deep autoencoder for audio and video modalities

% http://papers.nips.cc/paper/4683-multimodal-learning-with-deep-boltzmann-machines.pdf
% Combines keywords with images in embedding space, using separate encoders for each modality.

% https://ieeexplore.ieee.org/abstract/document/7293666
% Mapping between 2D and 3D learned via multimodal embedding

% https://journalofbigdata.springeropen.com/track/pdf/10.1186/s40537-016-0043-6
% General survey of what transfer learning is. Relatively old (2016)

% https://arxiv.org/pdf/1806.06176.pdf
% *** This has almost exact same idea that we have, by having a "multimodal discriminative factors" that gets shared across all modalities and modality-specific generative factors
% \fi


     %Each candidate contains the post itself and all comment trees. Specifically, the post contains link, title, post date and time\footnote{In Unix time}, number of views, ups, downs, points, comments count, favorite count, and tags, along with images and videos, plus any descriptions they have. Each comment in post's comment trees contains \textcolor{red}{its own ID, parent ID,} content, ups, downs, points, and platform, where the content can be text or image/video.

    %Our dataset contains more than 603k candidates. Table \ref{tab:raw_ds_statistics} shows general statistics over the dataset. Figure \ref{fig:raw_dataset_distributions} illustrates some of the distributions.
    % Distributions of raw data across time are shown in Figure \ref{fig:date_distribution}. We also plot distribution of number of views in Figure \ref{fig:views_distribution}. 
    %For date distribution specifically, it could be noticed that there are several gaps in 2019. This is due to initial testing of the scraper script using some dates in 2019. The irregularities in terms of number of posts per day are caused by various difficulties encountered during scraping, including Imgur server errors, network errors, faulty website addresses, and errors from packages for processing images. %\textcolor{red}{(image/url not found, segfault, server error, service temporarily unavailable, cannot be properly cropped by OpenCV, not found for url, failed to establish new connection, Invalid PNG signature 0x1F8B080000000000. No JPEG data found in image, 404 Client Error: Not Found for url: http://www.gsgoehl.de/img/natur/butt013.jpg. Core Dump/Segfault)}
 
 
    % \begin{figure*}[h]
    %   \centering
    %     \includegraphics[width=1\textwidth]{images/post_date_distribution.png}
    %   \caption{Date distribution. Only limited amount of data are available before late 2015.}
    %   \label{fig:date_distribution}
    % \end{figure*}
    
    % %\begin{figure*}[h]
    % %  \centering
    % %    \includegraphics[width=1\textwidth]{images/tags_distribution.png}
    % %  \caption{Tags distribution for \DS Dataset. There are 77451 different tags in total. For rendering purposes the plot only shows the first 1200 of them. The entire distribution is heavily concentrated in the first 100 tags and has a long tail. The red line correspond to the $1000^{th}$ tag, which covers 76.09\% of tags usage throughout all posts. Best viewed in large}
    % %  \label{fig:tags_distribution}
    % %\end{figure*}    
    
    % \begin{figure*}[h]
    %   \centering
    %     \includegraphics[width=1\textwidth]{images/raw_dataset_views_distribution.png}
    %     \includegraphics[width=1\textwidth]{images/raw_dataset_views_distribution_2.png}
    %   \caption{\todo{Which one seems better? top or bottom} Views distribution for our Dataset. Both bar plots contain of 2000 bins with bin size 100. For rendering purposes only posts with less than 200,000 views are shown, which includes 89.22\% of posts. Best viewed in large.
    %  % For training split, 227443 examples in total, Retained 216569, Removed 10874. range 0 to 400,000 and 2,000 bins. so each bin has range 200 views. Plotted only some posts as there are extreme outliers (https://imgur.com/a/RrygZ has 36,019,622,132 Views, far from the rest of the distribution)
    %   }
    %   \label{fig:views_distribution}
    % \end{figure*}



%     \begin{figure*}[h]
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000397_999.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000397_001.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000397_002.png}  
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000397_003.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000397_004.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000397_005.png}
%     \end{subfigure}
%     \caption*{
% \footnotesize 
% \textbf{title}          : How people survived the 80's \\
% \textbf{top comment}    : I used to cover entire rooms with carefully placed green army men in preparation for epic battles. Then I just looked at them and cleaned up \\
% \textbf{description}    : If you got to have a birthday this was the place to go! Who doesn't like ball pits, arcade games, and terrifying robots. \\
% \scriptsize
% \textbf{datetime}       : 1474898934 \quad
% \textbf{views}          : 44,013 \quad
% \textbf{ups}            : 1094 \quad
% \textbf{downs}          : 42 \quad
% \textbf{points}         : 1052 \quad
% \textbf{score}          : 1073 \quad
% \textbf{comment count}  : 74 \quad
% \textbf{favorite count} : 302 \quad
% \textbf{tags}           : ['storytime'] \\
%     }
% %     \begin{subfigure}{.16\textwidth}
% %       \centering
% %       \includegraphics[width=\linewidth]{images/examples/000530_999.png}
% %     \end{subfigure}
% %     \begin{subfigure}{.16\textwidth}
% %       \centering
% %       \includegraphics[width=\linewidth]{images/examples/000530_001.png}
% %     \end{subfigure}
% %     \begin{subfigure}{.16\textwidth}
% %       \centering
% %       \includegraphics[width=\linewidth]{images/examples/000530_002.png}  
% %     \end{subfigure}
% %     \begin{subfigure}{.16\textwidth}
% %       \centering
% %       \includegraphics[width=\linewidth]{images/examples/000530_003.png}
% %     \end{subfigure}
% %     \begin{subfigure}{.16\textwidth}
% %       \centering
% %       \includegraphics[width=\linewidth]{images/examples/000530_004.png}
% %     \end{subfigure}
% %     \begin{subfigure}{.16\textwidth}
% %       \centering
% %       \includegraphics[width=\linewidth]{images/examples/000530_005.png}
% %     \end{subfigure}
% %     \caption*{
% % title          : This Week on DeviantArt - Jul 22
% % datetime       : 1500735845
% % views          : 67405
% % ups            : 940
% % downs          : 44
% % points         : 896
% % score          : 929
% % comment count  : 15
% % favorite count : 614
% % tags           : ['creativity']
% % top comment    : I misread #1 as collateral mercy... I like my version better...
% % description    : (31) Hello
% % Artist: Radittz
% % Source: http://deviantart.com/art/Hello-692888309
% %     }
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000751_999.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000751_001.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000751_002.png}  
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000751_003.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000751_004.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/000751_005.png}
%     \end{subfigure}
%     \caption*{
% \footnotesize 
% \textbf{title}          : Made an Arch reactor for my nephew's Iron Man Halloween costume. \\
% \textbf{top comment}    : Arc \\
% \textbf{description}    : I got my nephew the Iron Man helmet the Christmas prior which gave the costume a big step up. I mailed my sister the arc reactor and she took it from there to put it on the suit. Happy Halloween. \\
% \scriptsize
% \textbf{datetime}       : 1477713120 \quad
% \textbf{views}          : 42,318 \quad
% \textbf{ups}            : 1006 \quad
% \textbf{downs}          : 33 \quad
% \textbf{points}         : 973 \quad
% \textbf{score}          : 994 \quad
% \textbf{comment count}  : 24 \quad
% \textbf{favorite count} : 167 \quad
% \textbf{tags}           : ['Halloween'] \\
%     }
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001365_999.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001365_001.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001365_002.png}  
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001365_003.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001365_004.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001365_005.png}
%     \end{subfigure}
%     \caption*{
% \footnotesize
% \textbf{title}          : 5 things I didn't know I wanted until now.... \\
% \textbf{top comment}    : I feel robbed and cheated by this. \\
% \textbf{description}    : For those that like to keep the crunch in their cereal, here’s the bowl to get. It separates the milk from the cereal, so all you have to do is dunk the cereal into the milk right before you eat it. You’ll get all of the flavor with none of the sog. \\
% \scriptsize
% \textbf{datetime}       : 1449907198 \quad
% \textbf{views}          : 141,775 \quad
% \textbf{ups}            : 5640 \quad
% \textbf{downs}          : 513 \quad
% \textbf{points}         : 5127 \quad
% \textbf{score}          : 5197 \quad
% \textbf{comment count}  : 166 \quad
% \textbf{favorite count} : 2049 \quad
% \textbf{tags}           : ['funny', 'mcbs'] \\
%     }
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001523_999.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001523_001.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001523_002.png}  
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001523_003.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001523_004.png}
%     \end{subfigure}
%     \begin{subfigure}{.16\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{images/examples/001523_005.png}
%     \end{subfigure}
%     \caption*{
% \footnotesize
% \textbf{title}          : Secret santa really blew me away! \\
% \textbf{top comment}    : That is freaking adorable \\
% \textbf{description}    : Wow!  A whole porg?! \\
% \scriptsize
% \textbf{datetime}       : 1545068736 \quad
% \textbf{views}          : 105,549 \quad
% \textbf{ups}            : 1853 \quad
% \textbf{downs}          : 102 \quad
% \textbf{points}         : 1751 \quad
% \textbf{score}          : 1803 \quad
% \textbf{comment count}  : 43 \quad
% \textbf{favorite count} : 132 \quad
% \textbf{tags}           : ['secret santa']
%     }
%     \caption{Sample posts. For rendering purposes we only display a single image (first column from left) and  five of the frames from a single video out of potentially multiple images/videos in each post, and only display a single text comment out of multiple comment trees. \todo{make this into a vertical table}}
%     \label{fig:sample_post}
%     \end{figure*}
    
        % To visualize the distribution of all posts's images, we use ImageNet pre-trained ResNet152 to predict class labels for images. We show the distribution of class results in Figure \ref{fig:ImageNet_image}. 

    
    
    % \begin{figure*}[h]
    %   \centering
    %     \includegraphics[width=\textwidth]{images/train_image_distribution.png}
    %     \includegraphics[width=\textwidth]{images/val_image_distribution.png}
    %   \caption{\VUN ImageNet Classification results distribution for images (Top: Train split. Bottom: Validation split). The distribution peaks at class 916, which correspond to 'web site, website, internet site, site'. \todo{Consider updating this figure to make it more useful/add something to the figure}}
    %   \label{fig:ImageNet_image}
    % \end{figure*}
    
    % For ImageNet classification, we randomly select one video from each post, evaluate all its frames using pre-trained ResNet152, and average the output scores and apply softmax to obtain final class label. If there is no video for that post, we use randomly sampled image instead. We show the distribution of class results in Figure \ref{fig:ImageNet_video}.
    
    % \begin{figure*}[h]
    %   \centering
    %     \includegraphics[width=\textwidth]{images/train_video_distribution.png}
    %     \includegraphics[width=\textwidth]{images/val_video_distribution.png}
    %   \caption{ImageNet Classification results distribution for videos (Top: Train split. Bottom: Validation split).}
    %   \label{fig:ImageNet_video}
    % \end{figure*}
    
    %    We instantiate instances of an exact same decoder as points ratio and views decoders. Similar to Tags decoder, the contextual embedding is first flattened across the encoder dimension, then gets passed into a single layer fully connected network to predict  points ratio.

%\subsection{Language decoder}
%    For each of the language modalities, we instantiate an instance of the exact same decoder. The decoder is a 100 units, 2 layers LSTM, with hidden size equal to vocabulary size of predicted words
    
    
%    \todo{Update this section!}
    
    
    
%    whose basic block is shown in \todo{Add a plot for language decoder as it's a bit more involved}. Each block takes in the previous hidden state, contextual embedding, and word embedding of the previous two words to generate a new hidden state and a score vector. The index of the maximum value in the score vector correspond to the index of the predicted word. 
    
%    To build the word embedding, we use space separation to obtain unique words in a given language modality, and selected the top 20,000 words as our vocabulary. We trained a 1024-dimension word embedding based on these words. 

    
    
    
    
    %To accommodate for an early release, we run experiments only on tags\footnote{Trained based a subset of full dataset consisting of 95K training, 11K validation, and 11K test} and points ratio as decoders. For tags, we use F1 score as evaluation metrics and Binary Cross Entropy loss as loss function. We also plot presence matrix and prediction accuracies\footnote{Since ground truth for tags is extremely sparse, true negatives are ignored and only true positives are taken into account for accuracy calculation, with 0.5 as cutoff threshold} to better visualize our results. For points ratio, we use Mean Squared Error loss as loss function.
    
    %It can also be observed that there exists significant fluctuations for training loss in Figure \ref{loss:com2pr}. We speculate that the uneven loss terrain which caused stochastic gradient descent to behave in such uncanny way implies the richness and complexity of language that is uniquely found in comments.
    
    %\subsection{Tags decoder}
%    The contextual embedding is first flattened across the encoder dimension, then gets passed into a single layer fully connected network to predict tags. 


    

% \subsubsection{AQ image to points ratio (From exp01)}
% Good
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/006.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/015.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/027.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/029.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/034.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/046.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/051.png
% best https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/062.png
% best https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/089.png
% best https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/099.png
% best https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/105.png
% best https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/110.png
% Bad
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/021.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/030.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/035.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/038.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/041.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/042.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/101.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_AQ/exp01/val/sample/109.png


% % \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/Points%20Ratio%20Loss%20Curves.png}{Loss Curve}
% Wrong data split!!!
% \begin{itemize}
%     \item Good 
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/002.png}{S1}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/022.png}{S2}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/064.png}{S3}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/066.png}{S4}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/084.png}{S5}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/107.png}{S6}
%     \item Bad 
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/005.png}{S1}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/046.png}{S2}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/067.png}{S3}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/081.png}{S4}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/088.png}{S5}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/103.png}{S6}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/114.png}{S7}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_AQ_visualizations/test/sample/115.png}{S8}
% \end{itemize}

% \subsubsection{BQ video to points ratio (From exp01)}
% Good
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/006/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/008/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/031/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/072/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/095/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/106/001.png
% best https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/111/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/119/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/123/001.png
% Bad
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/021/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/030/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/035/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/038/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/041/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/058/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/101/001.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_BQ/exp01/val/sample/109/001.png


% \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/Points%20Ratio%20Loss%20Curves.png}{Loss Curve}
% Wrong data split!!!
% \begin{itemize}
%     \item Good
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/022/001.png}{S1}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/035/001.png}{S2}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/039/001.png}{S3}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/052/001.png}{S4}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/072/001.png}{S5}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/113/001.png}{S6}
%     \item Bad
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/005/001.png}{S1}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/018/001.png}{S2}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/046/001.png}{S3}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/067/001.png}{S4}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/114/001.png}{S5}
%     \href{https://github.com/xuebofan/Experiment_visualizations/blob/master/visualizations/_FEB_18_2020_data_bs%3D128_BQ_visualizations/test/sample/115/001.png}{S6}
% \end{itemize}

% \subsection{CQ}
% Good
% https://github.com/xuebofan/visualizations/blob/master/_MAR_2_2020_data_bs%3D128_CQ/exp01/val/sample/060.png
% Bad
% https://github.com/xuebofan/visualizations/blob/master/_MAR_2_2020_data_bs%3D128_CQ/exp01/val/sample/006.png
% https://github.com/xuebofan/visualizations/blob/master/_MAR_2_2020_data_bs%3D128_CQ/exp01/val/sample/041.png
% https://github.com/xuebofan/visualizations/blob/master/_MAR_2_2020_data_bs%3D128_CQ/exp01/val/sample/087.png
% https://github.com/xuebofan/visualizations/blob/master/_MAR_2_2020_data_bs%3D128_CQ/exp01/val/sample/089.png


% \subsubsection{DQ}
% Good: 
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/004.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/010.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/032.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/087.png
% best https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/100.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/102.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/113.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/114.png
% Bad:
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/021.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/030.png
% worst  https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/035.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/038.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/041.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/058.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/101.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_DQ/exp01/val/sample/109.png


% \subsection{EQ}
% Good:
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/016.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/033.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/034.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/054.png
% best https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/065.png
% best https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/117.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/120.png
% Bad:
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/021.png
% worst https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/035.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/038.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/041.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/042.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/056.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/058.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/069.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/071.png
% https://github.com/xuebofan/visualizations/blob/master/_FEB_18_2020_data_bs%3D128_EQ/exp01/val/sample/101.png

    
    
    % \begin{figure*}[h]
    % \begin{subfigure}{.34\textwidth}
    %   \centering
    %   \includegraphics[width=\linewidth]{images/FEB_18_2020_data_bs=128_AQ.png}
    %   \caption{Image to points ratio \\ \quad $L_1$ norm: 0.02293}
    %   \label{loss:img2pr}
    % \end{subfigure}
    % \begin{subfigure}{.34\textwidth}
    %   \centering
    %   \includegraphics[width=\linewidth]{images/FEB_18_2020_data_bs=128_BQ.png}
    %   \caption{Video to points ratio \\ \quad $L_1$ norm: 0.02111}
    %   \label{loss:vid2pr}
    % \end{subfigure}
    % \begin{subfigure}{.34\textwidth}
    %   \centering
    %   \includegraphics[width=\linewidth]{images/MAR_2_2020_data_bs=128_CQ.png}
    %   \caption{Description to points ratio \\ \quad $L_1$ norm: \todo }
    %   \label{loss:des2pr}
    % \end{subfigure}
    % \begin{subfigure}{.33\textwidth}
    %   \centering
    %   \includegraphics[width=\linewidth]{images/FEB_18_2020_data_bs=128_DQ.png}
    %   \caption{Title to points ratio \\ \quad $L_1$ norm: 0.02314}
    %   \label{loss:tit2pr}
    % \end{subfigure}
    % \begin{subfigure}{.33\textwidth}
    %   \centering
    %   \includegraphics[width=\linewidth]{images/FEB_18_2020_data_bs=128_EQ.png}
    %   \caption{Top comment to points ratio \\ \quad $L_1$ norm: 0.02578}
    %   \label{loss:com2pr}
    % \end{subfigure}
    % \begin{subfigure}{.33\textwidth}
    %   \centering
    %   \includegraphics[width=\linewidth]{images/MAR_31_2020_data_bs=128_ABCDEQ.png}
    %   \caption{All encoders to points ratio \\ \quad $L_1$ norm: \todo}
    %   \label{loss:all2pr}
    % \end{subfigure}
    % \caption{Loss curves for various experiments \todo{Should I include the result for test loss, as that partition is not released?}}
    % \label{fig:loss_curves}
    % \end{figure*}
    
        % \begin{table*}[h]
    %     \centering
    %     \begin{tabular}{|c|c|c|c|c|c|c|c|}
    %     \hline
    %       & & \multicolumn{3}{c|}{Top Comment Length per post} & \multicolumn{3}{c|}{Top Comment perplexity}\\
    %       \cline{3-8}
    %      & Number of Unique words & Mean & Median & StdDev & Mean & Median & StdDev \\
    %      \hline
    %      Train & 24,634 & 15.0530 & 13 & 8.8256 & 98.2056 & 80.0849 & 573.3582\\
    %      Validation & 17,533 & 15.0445 & 13 & 8.8323 & 59.2658 & 52.5042 & 36.6173\\
    %      \hline
    %     \end{tabular}
    %     \caption{Statistics over top comment}
    %     \label{tab:comment_statistics}
    % \end{table*}
    
        % \begin{table*}[h]
    %     \centering
    %     \begin{tabular}{|c|c|c|c|c|c|c|c|}
    %     \hline
    %      & & \multicolumn{3}{c|}{Title Length per post} & \multicolumn{3}{c|}{Title perplexity}\\
    %      \cline{3-8}
    %      & Number of Unique words & Mean & Median & StdDev & Mean & Median & StdDev \\
    %      \hline
    %      Train & 23,519 & 8.2005 & 7 & 6.2142 & 93.4751 & 71.3228 & 90.3729\\
    %      Validation & 15,286 & 8.1934 & 7 & 6.2425 & 53.4291 & 43.5758 & 45.3677\\
    %      \hline 
    %     \end{tabular}
    %     \caption{Statistics over titles}
    %     \label{tab:title_statistics}
    % \end{table*}
    
        % Given the multimodal nature of the dataset, we propose the concept of ``Multi-modal encoder'' \CN, which extracts and merges semantics information from various vision and language encoders and produces an output that can be used by various decoders. A graphical illustration of our model can be found in Figure \ref{model_plot}. Note that for illustration purposes while some of the language modalities may appear as both input and output simultaneously, in experiments they can only be either input or output.
        
            
        % \begin{table*}[h]
    %     \centering
    %     \begin{tabular}{|c|c|c|c|c|c|c|c|}
    %     \hline
    %      & & \multicolumn{3}{c|}{Descriptions per post} & \multicolumn{3}{c|}{Descriptions perplexity}\\
    %       \cline{3-8}
    %      & Number of Unique words & Mean & Median & StdDev & Mean & Median & StdDev \\
    %      \hline
    %      Train & 26,216 & 1.2964 & 0 & 5.6711 & 39.3146 & 1.4444 & 130.3231\\
    %      Validation & 18,911 & 1.2449 & 0 & 5.4420 & 22.4406 & 1.4369 & 62.3815 \\
    %      \hline
    %     \end{tabular}
    %     \caption{Statistics over descriptions}
    %     \label{tab:des_statistics}
    % \end{table*}

    
    % \begin{table}[h]
    %     \centering
    %     \begin{tabular}{|c|c|c|c|}
    %     \hline
    %       & \multicolumn{3}{c|}{Number of videos per post} \\
    %       \cline{2-4}
    %      & Mean & Median & StdDev \\
    %      \hline
    %      Train & 0.6219 & 0 & 3.5864\\
    %      Validation & 0.6302 & 0 & 3.6238\\
    %      \hline
    %     \end{tabular}
    %     \caption{Statistics over videos}
    %     \label{tab:vid_statistics}
    % \end{table}    
    
        \begin{table}[h]
        \centering
        \begin{tabular}{|c|c|c|c|c|}
        \hline
         & & \multicolumn{3}{c|}{Points Ratio} \\
         \cline{3-5}
         & Examples & Mean & Median & StdDev \\
         \hline
         Train & 324,888 & 0.9567 & 0.9665 & 0.0370 \\
         Validation & 40,448 & 0.9571 & 0.9667 & 0.0366 \\
         \hline
        \end{tabular}
        \caption{Statistics over points ratio}
        \label{tab:points_ratio_statistics}
    \end{table}
    
    
    
DS name keywords : multi-modality, language, vision, Berkeley, 

experiment results for ABQ, CDEQ, ABCDEQ

% Major notes on the paper: You can summarize Fig 5. in a table
%There's no reason to have loss curves
%Figure 3 still needs some more visual diverse samples (it's ok to cherry-pick a bit), and the captions for figure 3 need to look a bit nicer.
%Maybe sample the videos at a slightly longer frame-rate? It seems like you're sampling frames that are very close together
%and they look visually identical
% For fig. 5 - you don't need to include test loss
% You need to get things under 8 pages (I think, not including references) - so combining tables 5,6,7 and 7 might be able to do this
%Let's leave out "Core-Knowledge" for now - I think that is mostly confusing to people who don't have the background. Instead - let's call it a multi-modal encoder
% Table 3 has problems with formatting
As far as dataset names, you created the dataset, so you should pick the name!
% Let's keep both plots for figure 2, but make them 1/2 page width
% It might even be better to make them 1/3 page width with Figure 1

%Table 2 is somewhat useless - you can probably save space just by saying this information in the text
%Table 1 is great
%Though for table 1, the # of comment tree leaves, and mean/media/std depth probably belong in their own table
%A "comment-statistics" table
You also seem to be missing a lot of articles such as "the" or "an" in the text. Passing the text through "grammarly" can help


\DS = dataset refers to full dataset

% views distribution: only plot 90\% data, and say the rest will be incomprehensible 
% views distribution and date distribution increase font size

% save all losses for eval
% using mean of points ratio as the dummy predicted result, compute l_1 and l_2 distance for all eval instances, along with std
% t test for all encoders pairwise: each of the encoder losses against other encoder losses 
% sample for CDEQ and ABCDEQ

Email to mul.workshop.cvpr2020@gmail.com for submission


    \begin{table}[h]
        \footnotesize
        \centering
        \begin{tabular}{|c|c|c|c|}
            \hline
            & Train & \multicolumn{2}{c|}{Validation} \\
            \cline{2-4}
            Encoder(s) used & $L_2$ distance & $L_1$ distance & $L_2$ distance \\
            \hline
            Baseline(Using Mean train Points ratio) & &  & 0.001389 \\
            \hline
            Image & 4.2330e10-4 & 0.02293 & 1.4751e10-3 \\
            \hline
            Video &  & 0.02111 & 1.3098e10-3\\
            \hline
            Description & 1.0412e10-3 & 0.02397 & 1.5856e10-3 \\
            \hline
            Title & 1.4164e10-3 & 0.02314 & 1.3697e10-3 \\
            \hline
            Top comment & 2.2003e10-4 & 0.02578 & 1.7461e10-3 \\
            \hline
            Image and video & 2.6951e10-4 & 0.02369 & 1.5055e10-3 \\
            \hline
            Description, title, & 1.0948e10-4 & 0.02428 & 1.5964e10-3 \\
            and top comment & & & \\
            \hline
            All encoders & 4.0354e-05 & 0.02323 & 1.3379e10-3\\
            \hline
        \end{tabular}
        \caption{Points ratio validation losses after 100 epochs \todo{Do we need std for this?}}
        \label{tab:losses}
    \end{table}


    \begin{table*}[h]
        \centering
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
            \hline
            & Image & Video & Description & Title & Top comment & (Vision) Image and video & (Language) Description, title and top comment & All encoders \\
            \hline
            Image & 0.0000 & 3.0540 & -1.8596 & 1.9533 & -4.9251 & -0.6017 & -2.4832 & 2.7395 \\
            \hline
            Video & -3.0540 & 0.0000 & -4.7428 & -1.0345 & -7.9120 & -3.7266 & -5.4686 & -0.5601 \\
            \hline
            Description & 1.8596 & 4.7428 & 0.0000 & 3.6722 & -2.8397 & 1.3311 & -0.5283 & 4.5535 \\
            \hline
            Title & -1.9533 & 1.0345 & -3.6722 & 0.0000 & -6.7358 & -2.5847 & -4.3432 & 0.5680 \\
            \hline
            Top comment & 4.9251 & 7.9120 & 2.8397 & 6.7358 & 0.0000 & 4.4455 & 2.3888 & 7.9676 \\
            \hline
            (Vision) Image and video & 0.6017 & 3.7266 & -1.3311 & 2.5847 & -4.4455 & 0.0000 & -1.9503 & 3.4666 \\
            \hline
            (Language) Description, title and top comment & 2.4832 & 5.4686 & 0.5283 & 4.3432 & -2.3888 & 1.9503 & 0.0000 & 5.3397 \\
            \hline
            All encoders & -2.7395 & 0.5601 & -4.5535 & -0.5680 & -7.9676 & -3.4666 & -5.3397 & 0.0000 \\
            \hline
        \end{tabular}
        \caption{\todo{This is a new table} T-statistics \textcolor{red}{using eval losses from each of the experiments}}
        \label{tab:t_statistics}
    \end{table*}
    

    \begin{table*}[h]
        \centering
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
            \hline
            & Image & Video & Description & Title & Top comment & (Vision) Image and video & (Language) Description, title and top comment & All encoders \\
            \hline
            Image & 0.0000 & 0.0023 & 0.0629 & 0.0508 & 0.0000 & 0.5474 & 0.0130 & 0.0062 \\
            \hline
            Video & 0.0023 & 0.0000 & 0.0000 & 0.3009 & 0.0000 & 0.0002 & 0.0000 & 0.5754 \\
            \hline
            Description & 0.0629 & 0.0000 & 0.0000 & 0.0002 & 0.0045 & 0.1832 & 0.5973 & 0.0000 \\
            \hline
            Title & 0.0508 & 0.3009 & 0.0002 & 0.0000 & 0.0000 & 0.0098 & 0.0000 & 0.5701 \\
            \hline
            Top comment & 0.0000 & 0.0000 & 0.0045 & 0.0000 & 0.0000 & 0.0000 & 0.0169 & 0.0000 \\
            \hline
            (Vision) Image and video & 0.5474 & 0.0002 & 0.1832 & 0.0098 & 0.0000 & 0.0000 & 0.0511 & 0.0005 \\
            \hline
            (Language) Description, title and top comment & 0.0130 & 0.0000 & 0.5973 & 0.0000 & 0.0169 & 0.0511 & 0.0000 & 0.0000 \\
            \hline
            All encoders & 0.0062 & 0.5754 & 0.0000 & 0.5701 & 0.0000 & 0.0005 & 0.0000 & 0.0000 \\ 
            \hline
        \end{tabular}
        \caption{\todo{This is a new table} P-values for T-statistics \textcolor{red}{using eval losses from each of the experiments}}
        \label{tab:p_values_for_t_statistics}
    \end{table*}
    
    
    % We demonstrate the general structure of our model in Figure \ref{model_plot}. Specifically, our model takes in any combinations of [image, video, description, title, top comment] and tries to predict points ratio\footnote{Computed as ups/(ups + downs)}. Details about encoders, decoders, and Multi-modal encoder are discussed in the following sections.
    %We demonstrate the general structure of our model in Figure \ref{model_plot}. Specifically, our model takes in any combinations of [image, video, description, title, top comment] and tries to predict any combinations of [tags\footnote{Constructed as 1000 dimension k-hot vector}, points ratio\footnote{Computed as ups/(ups + downs)}, description, title, top comment, views\footnote{Normalized against a threshold value, which is chosen to be 200,000 number of views. The maximum normalized value is capped at 5. These measures are taken to eliminate extreme values from outliers}], except for cases where a given modality is in both encoder and decoder. Details about encoders, decoders, and Core-Knowledge Module are discussed in the following sections.
    
    
    % To accommodate for an early release, we only run experiments\footnote{All experiments are performed over slightly smaller versions of the released dataset} that predicts points ratio. Specifically, using points ratio as the only decoder, experiments include using any of the encoders, image and video encoders, description, title and top comment encoders, and all of the encoders\footnote{It should be noted that there exists a large combinations of encoders and decoders that can be used for different experiments}.
    
    % \subsection{Relationship between platform and comments}    
%     A less well explored direction is understanding the relationship between platform\footnote{Can be `iphone', `android', or `desktop'} and comments
    
%     While performing some basic statistics would show changes, if any, of platform usage through 6 years of time, we hypothesis that differences in platform usage affects varies parts of the comment, including likelihood of responding with images and videos, 
    
    
%     such as style of the post (e.g. number of videos, length of the description, time at which the post gets posted, etc.) or responses in the comment. It is possible that certain types of posts or responses are more likely to be found in one platform than the other.
    
    
    
%     Given the information on the platform that people used, it is also possible to investigate variations in posts due to differences in platform used

    % Aside from the pre-trained models, while language encoder is using Transformers, the rest of the encoders and decoders and the multi-modal encoder are only fully connected networks. Clearly more advanced models can be utilized in the encoder, decoder, or multi-modal encoder to improve not only the performance of 1 to 1 encoder-decoder experiments, but also 1 to k, k to 1, and k to k encoders-decoders experiments. This requires tailored encoders and decoders networks, along with a strong multi-modal encoder that is capable of extracting contextual information from various vision and language encoders. We believe our dataset is big enough such that a reasonably large and complex model will perform better and will not over-fit.
    %The complexity of the model, along with the size of the embedding output, should align with the complexity of the input. 
    %more advanced networks for each modality, including a multi-modal encoder that condenses information through all modalities. 
    %Currently the image embedding takes the most drive space, which is even larger than the embedding size of video frames. This shouldn't happen as video inherently contains more information than image. More advanced networks should be applied over videos, otherwise image embedding size should be reduced. On the other hand, besides the Transformer model we used as text encoders, all other parts of the model are basically fully connected layers. They worked reasonably well when we do single encoder to single decoder training, but they perform poorly when trying to generalize to multiple encoders or decoders. Future work should not only increase the complexity of both encoder and decoder networks, but also come up with a Core-Knowledge model that is capable of learning contextual information from visual and linguistic modalities.

==> presentation_model.tex <==
\begin{figure}
        %%%%%%%%%% Credit http://www.texample.net/tikz/examples/neural-network/
        \def\layersep{1.5cm}
        \begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
            \tikzstyle{every pin edge}=[<-,shorten <=1pt]
            \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
            \tikzstyle{encoder}=[neuron, fill=green!50];
            \tikzstyle{unused_encoder}=[neuron, fill=green!15];
            \tikzstyle{decoder}=[neuron, fill=red!50];
            \tikzstyle{unused_decoder}=[neuron, fill=red!8];
            \tikzstyle{multi-modal encoder}=[neuron, fill=blue!50];
            \tikzstyle{annot} = [text width=5em, text centered]
        
            % Draw the encoder nodes
            \node[encoder, pin=left:Image] (E-1) at (0,-1) {};
            \node[encoder, pin=left:Video] (E-2) at (0,-2) {};
            \node[encoder, pin=left:Title] (E-3) at (0,-3) {};
            \node[encoder, pin=left:Description] (E-4) at (0,-4) {};
            \node[encoder, pin=left:Comment] (E-5) at (0,-5) {};
            \node[unused_encoder, pin=left:Date] (E-6) at (0,-6) {};
        
            % Draw the multi-modal encoder nodes
            \foreach \name / \y in {1,...,1}
                \path[yshift=0.0cm]
                    node[multi-modal encoder] (C-1) at (\layersep,-3 cm) {};
        
            % Draw the decoder node
            \node[unused_decoder,pin={[pin edge={->}]right:Tags}] (D-1) at (2 * \layersep,-1){};
            \node[unused_decoder,pin={[pin edge={->}]right:Points ratio}] (D-2) at (2 * \layersep,-2){};
            \node[decoder,pin={[pin edge={->}]right:Points ratio}] (D-3) at (2 * \layersep,-3){};
            \node[unused_decoder,pin={[pin edge={->}]right:Description}] (D-4) at (2 * \layersep,-4){};
            \node[unused_decoder,pin={[pin edge={->}]right:Comment}] (D-5) at (2 * \layersep,-5){};
        
            % Connect every node in the input layer with every node in the
            % hidden layer.
            \foreach \source in {1,...,6}
                \foreach \dest in {1,...,1}
                    \path (E-\source) edge (C-\dest);
        
            % Connect every node in the hidden layer with the output layer
            \foreach \source in {1,...,1}
                \foreach \dest in {1,...,5}
                    \path (C-\source) edge (D-\dest);
        
            % Annotate the layers
            \node[annot,above of=C-1, node distance=1.5cm] (hl) {multi-modal encoder};
            \node[annot,above of=E-1, node distance=1cm] {Encoders};
            \node[annot,above of=D-1, node distance=1cm] {Decoders};
        \end{tikzpicture}
        \caption{Illustration of our model}
        \label{fig:model_plot}
    \end{figure}

